Extended Abstract: Motion Planners Learned from Geometric Hallucination

Learning motion planners to move robot from one point to another within an obstacle-occupied space in a collision-free manner requires either an extensive amount of data or high-quality demonstrations. This requirement is caused by the fact that among the variety of maneuvers the robot can perform, it is difficult to find the single optimal plan without many trial-and-error or an expert who is already capable of doing so. However, given a plan performed in obstacle-free space, it is relatively easy to find an obstacle geometry, where this plan is optimal. We consider this "dual" problem of classical motion planning and name this process of finding appropriate obstacle geometry as hallucination. In this work, we present two different approaches to hallucinate (1) the most constrained and (2) a minimal obstacle space where a given plan executed during an exploration phase in a completely safe obstacle-free environment remains optimal. We then train an end-to-end motion planner that can produce motions to move through realistic obstacles during deployment. Both methods are tested on a physical mobile robot in real-world cluttered environments.

==> content/experiments.tex <==
\section{EXPERIMENTS}
\label{sec::experiments}
Simulated and physical experiments are conducted to validate our hypothesis that HLSD technique can achieve at least similar, or even better performance (faster, smoother, safer) than classical method and the original LfH with runtime hallucination. In our experiments, we use a Clearpath Jackal robot, a four-wheeled, differential-drive, Unmanned Ground Vehicle (UGV), running Robot Operating System (ROS) \texttt{move\textunderscore base} navigation stack. Its DWA local planner is replaced with HLSD. Instead of requiring a high-resolution global path from the global planer (Dijkstra's), we only query a single local goal $c_g$ 1m away from the robot, and $c_c$ is the origin in the robot frame (orientation is ignored for simplicity). The UGV is equipped with a 720-dimensional LiDAR with a 270$^\circ$ field of view, and we clipped the maximum range to 1m to reduce the input space. The planning horizon $t$ is set to 1, i.e. only a single action $u_1 = \left(v_1, \omega_1\right)$ (linear and angular velocity) is produced for faster computation and better accuracy. $\pi_{rand}$ randomly picks a target $\left(\hat{v}, \hat{\omega}\right)$ pair and commands the robot to gradually reach that speed considering acceleration limit. After reaching $\left(\hat{v}, \hat{\omega}\right)$, $\pi_{rand}$ keeps that command with some probability or otherwise generates a new target command. We limit the output $v \in [0, 1.0]$m/s and $\omega \in [-1.57, 1.57]$rad/s. During training in a simulated open space, control inputs ($v$ and $\omega$) and robot configurations ($x$, $y$, and $\psi$) are recorded. Unlike the dataset collected by the original LfH~\cite{xiao2020toward}, which contains mostly $v=0.4$m/s, our dataset contains a variety of $v$ values. 12585 data points are collected in a 505s real-time simulation, including a rich variety of motions in an open space. We set \emph{sampling count} to 10 and $\alpha$ to 0.48. The $offset(\cdot)$ function linearly maps current $v$ in the range [0.3, 1.0]m/s to an offset value between [0, 1]m. Considering the fact that a real robot also needs to turn even in open space due to nonholonomic constraints, as opposed to an ideal point mass robot which does not, we also hallucinate $C_{obst}=\emptyset$ for configurations where $v>0.8$m/s. Considering highly constrained spaces, we additionally hallucinate the most constrained $C_{obst}^*$ for configurations where $v<0.3$m/s. So $|\mathcal{D}_{train}|$ is 12 times of $|\mathcal{D}_{raw}|$. We use the same three-layer neural network, with 256 hidden neurons and ReLU activation for each layer as in LfH. Training takes less than three minutes on a NVIDIA GeForce GTX 1650 laptop GPU. 

During deployment, we use a Model Predictive Control (MPC) model to check collision for safety. When collision is detected, the robot enters a two-phase recovery behavior: it first queries the global path immediate in front of the robot, and rotates to align the robot heading with the tangential direction of the global path. If this is still not safe, the robot backs up at $v=-0.2$m/s. Unlike the original LfH planner, HLSD does not require global path, for runtime hallucination and for the Turn in Place module to drive the robot out of out-of-distribution scenarios. Because our dataset contains varying $v \in [0, 1.0]$m/s, the original LfH speed modulation module to adapt mostly constant $v$ to real environments is not necessary either. The robot is able to react to the real obstacle configuration by using $f_{\theta}(\cdot)$ alone because $\mathcal{D}_{train}$ covers a wide range of distribution. 

\subsection{Simulated Experiments}
We first use a metric ground navigation benchmark dataset with 300 navigation environments~\cite{perille2020benchmarking} to compare (1) DWA, (2) original LfH trained on the mostly constant 0.4m/s dataset, (3) LfH trained on our varying speed 1.0m/s dataset, (4) HLSD trained on 0.4m/s dataset, and (5) HLSD trained on 1.0m/s dataset. To make a fair comparison, we double the max linear velocity of DWA to 1.0m/s, and also double the sampling rate for both linear and angular velocity (12 and 40, respectively). 

\xuesu{Simulation results here. }

\subsection{Physcial Experiments}
We also deploy the same set of local planners in a physical test course, five trials each (Fig. \ref{fig::physical} top). The results are shown in Tab. \ref{tab::results}. The complicated obstacle course causes DWA many recovery behaviors, and the robot takes a long average time with large variance to finish the traversal. LfH 0.4 and HLSD 0.4 are both able to successfully navigate the robot through, with similar traversal time. But note that LfH 0.4 requires a fine-resolution global path for hallucination during deployment and the Turn in Place module, while HLSD does not and only reacts to the real obstacles without any other extra components. LfH 1.0 fails every trial due to multiple collisions. The reason is learning from a dataset with varying speed and always hallucinating the most constrained spaces will cause ambiguity: the same most constrained C-space can map to different plans, which confuses the learner. Our HLSD 1.0 achieves the best performance both in terms of average time and standard deviation. HLSD deployment in a natural cluttered environment is shown in Fig. \ref{fig::physical} bottom. 

\begin{figure}[t]
  \centering
  \includegraphics[width=1\columnwidth]{content/figures/physical.png}
  \includegraphics[width=1\columnwidth]{content/figures/bwi.png}
  \caption{Physical Experiments (\url{https://tinyurl.com/hlsdnav})}
  \label{fig::physical}
\end{figure}

\begin{table}
\centering
\caption{Quantitative Results}
\begin{tabular}{cccccc}
\toprule
          & DWA & LfH 0.4 & LfH 1.0 & HLSD 0.4 & \textbf{HLSD 1.0} \\ 
\midrule
Time      &  78.8$\pm$10.0 & 67.0$\pm$4.4  & $\infty$ & 66.3$\pm$0.7 & \textbf{45.4$\pm$0.4}\\
\bottomrule
\end{tabular}
\label{tab::results}
\end{table}




==> content/related.tex <==
\section{RELATED WORK}
\label{sec::related}
This section presents related work in mobile robot navigation, using classical motion planning  and recent machine learning techniques. 

\subsection{Classical Motion Planning}
In terms of classical motion planning, mobile robot navigation is the problem of moving a robot from one point to another within an obstacle-occupied space in a collision free manner. Such planning usually happens in the robot Configuration Space (C-Space) \cite{latombe2012robot} and produces (asymptotically) optimal motion plans based on a predefined principle, such as maximum clearance, shortest path, or a combination thereof~\cite{lavalle2006planning}. These principles are represented in terms of C-space representation (e.g. cellular decomposition~\cite{lavalle2006planning}), global planning (e.g. A*~\cite{Hart1968}), and local planning. For example, the optimization-based Elastic Bands (E-Band) planner~\cite{quinlan1993elastic} uses repulsive forces generated from obstacles to deform and optimize an initial trajectory, primarily to achieve maximum clearance. The Dynamic Window Approach (DWA)~\cite{fox1997dynamic} samples feasible actions and score them based on a weighted score of distance to obstacle, closeness of following a global path, and the progress toward the goal. The new hallucination strategy proposed in this work assumes the planner learned from hallucinated training data primarily follows the shortest path principle. We leave hallucination strategies that follow the maximum clearance principle for future work. 

\subsection{Machine Learning for Navigation}


Despite decades of effort to develop classical autonomous navigation systems \cite{quinlan1993elastic, fox1997dynamic}, machine learning has been recently applied to create end-to-end planners with obstacle avoidance \cite{pfeiffer2017perception, muller2006off}, to enable terrain-based navigation \cite{wigness2018robot, siva2019robot}, to allow robots move around humans \cite{kretzschmar2016socially, chen2017socially}, to tune parameters for classical navigation systems \cite{xiao2020appld}, among others. All these learning methods require either an extensive body of training data, or relatively sparse data but of very high quality, usually from costly trial-and-error or human demonstrations, respectively. 

To address the difficulty in obtaining extensive or high-quality training data, self-supervised LfH \cite{xiao2020toward} collects training data in an obstacle-free environment with complete safety, and then learns a local navigation policy through synthetically projecting the most constrained C-space ($C_{obst}^*$) to the robot perception. However, LfH also requires hallucination of $C_{obst}^*$ during deployment. This hallucination ``on-the-fly'' requirement assumes a relatively fine-resolution global path is available. Furthermore, this previous work \cite{xiao2020toward} only works well when the linear velocity in the training set is mostly constant. This is due to the fact that the robot is always hallucinated to be navigating in the most constrained scenarios and the trained local planner is relatively conservative. Varying speeds in the same most constrained spaces will lead to ambiguity, as shown in our experiments (Section \ref{sec::experiments}). In this work, we eliminate the necessity of hallucination ``on-the-fly'', and therefore the requirement of an available fine-resolution global path. During sober deployment, the local planner only needs a single local goal point, along with the realistic, rather than hallucinated, perception. 
% To achieve sober deployment, we devise a more general hallucinated training technique than only hallucinating the most constrained C-spaces, so that the robot has seen as many different C-spaces as possible during training and does not need to be hallucinated during deployment. 
In addition, the novel hallucination technique also teaches the robot to vary its speed in response to the real environment, instead of the hallucinated most constrained spaces. 

